Enhancing the MILP/MIQCP-based Automatic Search for Differential-Linear Distinguishers of Simon-Like Ciphers

In this paper, we propose an improved method based on Mixed-Integer Linear Programming/Mixed-Integer Quadratic Constraint Programming (MILP/MIQCP) to automatically find better differential-linear (DL) distinguishers for the all members of Simon and Simeck block cipher families. To be specific, we first give the completely precise MILP model to describe the linear part, and explain how to utilize the general expressions of \textsf{Gurobi} solver to model the propagation of continuous difference for the middle part in a quite easy way. Secondly, in order to solve the MILP/MIQCP model in a reasonable time, we propose two heuristic strategies based on the divide-and-conquer idea to speed up the search process. Thirdly, we introduce the transforming technique, which exploits the clustering effect on DL trails, to improve the estimated correlation of the DL approximation. We apply our method to Simon and Simeck block cipher families. Consequently, we find the 14/17/21/26-round theoretical DL distinguishers of Simon32/48/64/96, which extend the previous longest ones of Simon32/48/96 by one round and Simon64 by two rounds, respectively. For Simeck, we do not explore longer distinguishers compared to the currently best results, but refresh all the results of Zhou et al. (the first work to automate finding DL distinguishers for Simon-like ciphers using MILP/MIQCP). Besides, in order to validate the correctness of these distinguishers, the experimental verifications are conducted on Simon32/Simeck32 and Simon48/Simeck48. The results show that our theoretical estimations on correlations are very close to the experimental ones, which can be regarded as a concrete support for the effectiveness of our method.

==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.46586/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

